3D Gaussian as a New Era: A Survey

3D Gaussian Splatting (3D-GS) has emerged as a significant advancement in the field of Computer Graphics, offering explicit scene representation and novel view synthesis without the reliance on neural networks, such as Neural Radiance Fields (NeRF). This technique has found diverse applications in areas such as robotics, urban mapping, autonomous navigation, and virtual reality/augmented reality, just name a few. Given the growing popularity and expanding research in 3D Gaussian Splatting, this paper presents a comprehensive survey of relevant papers from the past year. We organize the survey into taxonomies based on characteristics and applications, providing an introduction to the theoretical underpinnings of 3D Gaussian Splatting. Our goal through this survey is to acquaint new researchers with 3D Gaussian Splatting, serve as a valuable reference for seminal works in the field, and inspire future research directions, as discussed in our concluding section.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> Sections_Clean/Conclusion.tex <==
%\vspace{-0.5cm}
\section{Conclusions}\label{sec:Conclusion}

This paper offers a comprehensive and up-to-date overview of 3D-GS, summarizing existing methods and their applications. We begin by reviewing papers focused on optimizing 3D-GS for efficiencies, photorealism, costs, and physics. Subsequently, we systematically explore the five main applications of 3D-GS, including reconstructions, manipulations, generations, perceptions, and virtual humans. Lastly, we delve into challenges and potential future directions in this field. Additionally, we provide a comparative summary of methods in the Appendix, serving as a valuable resource for researchers in 3D vision and computer graphics.
%\vspace{-0.8cm}

==> Tables/dataset.tex <==
\begin{table*}[htbp]
\centering
\caption{List of commonly used datasets for 3D Gaussians.}
% \vspace{-0.3cm}
% \resizebox{\textwidth}{!}
{%
\begin{tabular}{>{\columncolor{C7!50}}l>{\columncolor{C6!50}}c>{\columncolor{C5!50}}c>{\columncolor{C4!50}}c>{\columncolor{C3!50}}c>{\columncolor{C2!50}}c>{\columncolor{C1!50}}c}
\toprule[1.5pt]
Dataset        & Year & Samples        & Classes & Type              & Representation       & Task                                \\ \midrule[1pt]
      &  &  &      &  &    &   
\\ \bottomrule[1.5pt]
\end{tabular}%
}\label{dataset}
\vspace{-0.3cm}
\end{table*}

==> Tables/dataset1.tex <==
\begin{table*}[htbp]
\centering
\caption{List of commonly used datasets for 3D Gaussians.}
\vspace{-0.3cm}
\resizebox{\textwidth}{!}
{%
\begin{tabular}{lcccccc}
\toprule[1.5pt]
\rowcolor{C7!50}Dataset        & Year & Samples        & Camera Views & Type              & Description      & Task                                \\ \midrule[1pt]
 
\rowcolor{C6!50}  Mip-NeRF 360~\cite{barron2022mip}  &CVPR'22  & 9 & 360 viewpoint     & Videos & \begin{tabular}[c]{@{}c@{}}Outdoor and indoor scene containing a complex \\central object or area with a detailed background  \end{tabular}  & \textcolor{blue}{Representation} \& Reconstruction \\
\rowcolor{C6!50}  Tanks and Temples~\cite{knapitsch2017tanks} & ToG'17 & 14 &   263-1107   & Videos & \begin{tabular}[c]{@{}c@{}}Ground-truth captured by high quality \\industrial laser scanner\end{tabular} & \textcolor{blue}{Representation} \& Reconstruction \\
\rowcolor{C6!50}  DeepBlending~\cite{hedman2018deep}  &TOG'18  & 19 &  12-418    & Images & \begin{tabular}[c]{@{}c@{}} Images with suicient variety of scene content \end{tabular}  & \textcolor{blue}{Representation} \& Reconstruction \\
\rowcolor{C6!50}  Plenoptic Video ~\cite{li2022neural} & CVPR'22 & 6 &   21   & Videos & \begin{tabular}[c]{@{}c@{}} Captured daily events with challenging scene motions\end{tabular} & \textcolor{blue}{Representation} \& Reconstruction \\
\rowcolor{C6!50}  D-Nerf~\cite{pumarola2021d}    & CVPR'21 & 8 & 360 viewpoint     &  Synthetic videos &   \begin{tabular}[c]{@{}c@{}} Animated
objects with complex geometries \\  and non-Lambertian materials \end{tabular}   & \textcolor{blue}{Representation} \& Manipulation \\
%\rowcolor{C6!50}    HyperNeRF~\cite{park2021hypernerf}  & SIGGRAPH Asia'21  &  &      &  &    & \textcolor{blue}{Representation} \\
\rowcolor{C6!50}    DyNeRF  & CVPR'22  & 6  & 20   & Videos &  \begin{tabular}[c]{@{}c@{}} Time-synchronized and calibrated multi-view \\  videos that covers challenging 4D scenes \end{tabular}  & \textcolor{blue}{Representation} \\
\rowcolor{C6!50}    NeRF-LLFF~\cite{mildenhall2019llff}  &  SIGGRAPH'19 & 8 & forward-facing views & images &  A subset of Real Iconic   & \textcolor{blue}{Representation} \\


\rowcolor{C5!50}  RealEstate10k~\cite{zhou2018stereo}  &ToG'18 & about 80k &  -   & Videos & \begin{tabular}[c]{@{}c@{}}Video clips on YouTube shot from a moving camera\end{tabular} & Reconstruction \\

\rowcolor{C5!50}  ACID~\cite{liu2021infinite}  &ICCV'21 & 765  &  -   & Videos & \begin{tabular}[c]{@{}c@{}} A dataset of aerial landscape videos\end{tabular} & Reconstruction \\

\rowcolor{C5!50}  ShapeNet~\cite{chang2015shapenet}  &2015 & about 60k  &  50   & Synthetic images & \begin{tabular}[c]{@{}c@{}} A richly-annotated, large-scale dataset of 3D shapes\end{tabular} & Reconstruction \\




\rowcolor{C4!50}  Tensor4D~\cite{shao2023tensor4d}    & CVPR'23 & 4 & 1, 4, 12     & Videos &   \begin{tabular}[c]{@{}c@{}}Dynamic half-body human videos by four\\ sparsely positioned, fixed RGB cameras\end{tabular}   & Manipulation \\
\rowcolor{C4!50}  Nerf-DS~\cite{pumarola2021d}    & CVPR'23 & 7 & 2 forward-facing views  & Videos &   Dynamic specular dataset   & Manipulation \\
\rowcolor{C4!50}  CoNeRF~\cite{kania2022conerf}    & CVPR'22 & 7 &  -  & Videos &   Real face scenes   & Manipulation \\
\rowcolor{C4!50}  InterHand2.6M~\cite{moon2020interhand2}    & ECCV'20 & 36 &  80-140 & Videos &   \begin{tabular}[c]{@{}c@{}} 2.6M labeled single and \\ interacting hand frames \end{tabular}   & Manipulation \\

\rowcolor{C3!50}   NVOS ~\cite{ren2022neural} & ICCV'22 & 7 &   20-62   &  Images &  \begin{tabular}[c]{@{}c@{}}  Real-world front-facing scenes with annotated object masks based on LLFF\end{tabular}  & Perception \\

\rowcolor{C3!50}    SPIn-NeRF ~\cite{mirzaei2023spin} & CVPR'23 & 10 & 100   & Images &  \begin{tabular}[c]{@{}c@{}} Real-world forward-facing
scenes with human annotated object masks \end{tabular}  & Perception \\

\rowcolor{C3!50}    LERF ~\cite{kerr2023lerf} & ICCV'23 & 13 & -   & Videos &  \begin{tabular}[c]{@{}c@{}} A mixture of in-the-wild and posed long-tail scenes\end{tabular}  & Perception \\

% \rowcolor{C3!50}  TUM RGB-D  ~\cite{sturm2012evaluating}& IROS'12 & 47 &  -  & Videos and Depths &  \begin{tabular}[c]{@{}c@{}} A large dataset containing RGB-D data and ground-truth data\end{tabular}  & Perception \\


\rowcolor{C3!50} Replica~\cite{straub2019replica}  &arXiv'19  & 18 &  -   &  Videos & \begin{tabular}[c]{@{}c@{}}  Highly photo-realistic 3D indoor scene dataset at room and building scale\end{tabular} & Perception \\

\rowcolor{C3!50} KITTI~\cite{geiger2012we}  &CVPR'12  & 22 &  -   &  Videos & \begin{tabular}[c]{@{}c@{}}   A city-scale dataset created for autonomous driving research\end{tabular} & Perception \\

\rowcolor{C2!50}    Objaverse 1.0~\cite{deitke2023objaverse} & CVPR'23 & 818k &   -   & 3D objects &  \begin{tabular}[c]{@{}c@{}} A large dataset of over 800K 3D models with descriptive captions, tags, and animations.\end{tabular} & Generation \\

\rowcolor{C2!50}    OmniObject3D~\cite{wu2023omniobject3d} & CVPR'23 & 6k &   -   & 3D objects &  \begin{tabular}[c]{@{}c@{}} Real-scanned 3D object captured with both 2D and 3D sensors, providing textured meshes, \\point clouds, multi-view rendered images, and multiple real-captured videos.\end{tabular}  & \begin{tabular}[c]{@{}c@{}} Generation \&  Perception \\ \& Reconstruction \end{tabular} \\

\rowcolor{C1!50}     People-Snapshot~\cite{alldieck2018video} & CVPR'18 & 24 &    1  & Videos &  \begin{tabular}[c]{@{}c@{}} Containing subjects captured with varying sets of garments \\ and with three different background scenes \end{tabular} & Virtual Humans \\

\rowcolor{C1!50}     DynaCap~\cite{habermann2021real} & ToG'21 & 5 &    50-101  & Videos &  \begin{tabular}[c]{@{}c@{}} Recording 5 subjects wearing different types of apparel \\ and performing a wide range of motions like "dancing"\end{tabular} & Virtual Humans \\

\rowcolor{C1!50}     ZJU-Mocap~\cite{peng2021neural} & CVPR'21 & 9 &    21  & Videos &  9 dynamic
human videos with 60 to 300 frames  & Virtual Humans \\

\rowcolor{C1!50}     THuman4~\cite{zheng2022structured} & CVPR'22 & 3 &    24  & Videos &  multi-view
human videos ranging from 2500 to 5000 frames & Virtual Humans \\

\rowcolor{C1!50}     NeuMan~\cite{jiang2022neuman} & ECCV'22 & 6 &    1  & Videos &  \begin{tabular}[c]{@{}c@{}} Monocular videos featuring a single individual \\ captured using a mobile phone \end{tabular} & Virtual Humans \\

\rowcolor{C1!50}     ActorsHQ~\cite{icsik2023humanrf} & arXiv'23 & 16 &    160  & Videos &  \begin{tabular}[c]{@{}c@{}} Containing 8 actors with casual clothing such as skirts or shorts\end{tabular} & Virtual Humans
\\ \bottomrule[1.5pt]
\end{tabular}%
}\label{dataset}
\vspace{-0.5cm}
\end{table*}

==> Tables/datasetV1.tex <==
\begin{table*}[htbp]
\centering
\caption{\textcolor{blue}{List of commonly used datasets for 3D Gaussians (``\#Number'' represents the number of 3D-GS papers that utilize this dataset).}}
\vspace{-0.4cm}
\resizebox{\textwidth}{!}
{%
\begin{tabular}{lccccccc}
\toprule[1.5pt]
\rowcolor{C7!50}Dataset        & Year & Samples        & Camera Views & Type              & Description   & Task    & \textcolor{blue}{\#Number}                              \\ \midrule[1pt]
 
\rowcolor{C6!50}  Mip-NeRF 360~\cite{barron2022mip}  &CVPR'22  & 9 & 360 viewpoint     & Videos & \begin{tabular}[c]{@{}c@{}}Outdoor and indoor scene containing a complex \\central object or area with a detailed background  \end{tabular} & \textcolor{blue}{Representation} \& Reconstruction  & \textcolor{blue}{49} \\

\rowcolor{C6!50}  Tanks and Temples~\cite{knapitsch2017tanks} & ToG'17 & 14 &   263-1107   & Videos & \begin{tabular}[c]{@{}c@{}}Ground-truth captured by high quality \\industrial laser scanner\end{tabular} & \textcolor{blue}{Representation} \& Reconstruction & \textcolor{blue}{34} \\

\rowcolor{C6!50}  DeepBlending~\cite{hedman2018deep}  &TOG'18  & 19 &  12-418    & Images & \begin{tabular}[c]{@{}c@{}} Images with suicient variety of scene content \end{tabular} & \textcolor{blue}{Representation} \& Reconstruction & \textcolor{blue}{18} \\

\rowcolor{C6!50}  Plenoptic Video~\cite{li2022neural} & CVPR'22 & 6 &   21   & Videos & \begin{tabular}[c]{@{}c@{}} Captured daily events with challenging scene motions\end{tabular} & \textcolor{blue}{Representation} \& Reconstruction & \textcolor{blue}{3} \\

\rowcolor{C6!50}  D-Nerf~\cite{pumarola2021d}    & CVPR'21 & 8 & 360 viewpoint     &  Synthetic videos &   \begin{tabular}[c]{@{}c@{}} Animated objects with complex geometries \\  and non-Lambertian materials \end{tabular}  & \textcolor{blue}{Representation} \& Manipulation  &  \textcolor{blue}{9} \\

\rowcolor{C6!50}    DyNeRF~\cite{li2022neural}  & CVPR'22  & 6  & 20   & Videos &  \begin{tabular}[c]{@{}c@{}} Time-synchronized and calibrated multi-view \\  videos that covers challenging 4D scenes \end{tabular}  & \textcolor{blue}{Representation} & \textcolor{blue}{3} \\

\rowcolor{C6!50}    NeRF-LLFF~\cite{mildenhall2019llff}  &  SIGGRAPH'19 & 8 & forward-facing views & images &  A subset of Real Iconic  & \textcolor{blue}{Representation} & \textcolor{blue}{11} \\

\rowcolor{C5!50}  RealEstate10k~\cite{zhou2018stereo}  &ToG'18 & about 80k &  -   & Videos & \begin{tabular}[c]{@{}c@{}}Video clips on YouTube shot from a moving camera\end{tabular} & Reconstruction  & \textcolor{blue}{3} \\

\rowcolor{C5!50}  ACID~\cite{liu2021infinite}  &ICCV'21 & 765  &  -   & Videos & \begin{tabular}[c]{@{}c@{}} A dataset of aerial landscape videos\end{tabular} & Reconstruction  & \textcolor{blue}{2} \\

\rowcolor{C5!50}  ShapeNet~\cite{chang2015shapenet}  &2015 & about 60k  &  50   & Synthetic images & \begin{tabular}[c]{@{}c@{}} A richly-annotated, large-scale dataset of 3D shapes\end{tabular} & Reconstruction & \textcolor{blue}{0} \\

\rowcolor{C4!50}  Tensor4D~\cite{shao2023tensor4d}    & CVPR'23 & 4 & 1, 4, 12     & Videos &   \begin{tabular}[c]{@{}c@{}}Dynamic half-body human videos by four\\ sparsely positioned, fixed RGB cameras\end{tabular}   & Manipulation & \textcolor{blue}{5} \\

\rowcolor{C4!50}  \textcolor{blue}{NeRF-DS}~\cite{pumarola2021d}    & CVPR'23 & 7 & 2 forward-facing views  & Videos &   Dynamic specular dataset & Manipulation  & \textcolor{blue}{2} \\

\rowcolor{C4!50}  CoNeRF~\cite{kania2022conerf}    & CVPR'22 & 7 &  -  & Videos &   Real face scenes   & Manipulation & \textcolor{blue}{1} \\

\rowcolor{C4!50}  InterHand2.6M~\cite{moon2020interhand2}    & ECCV'20 & 36 &  80-140 & Videos &   \begin{tabular}[c]{@{}c@{}} 2.6M labeled single and \\ interacting hand frames \end{tabular}  & Manipulation  & \textcolor{blue}{1} \\

\rowcolor{C3!50}   NVOS~\cite{ren2022neural} & ICCV'22 & 7 &   20-62   &  Images &  \begin{tabular}[c]{@{}c@{}}  Real-world front-facing scenes with annotated object masks based on LLFF\end{tabular}  & Perception  & \textcolor{blue}{1} \\

\rowcolor{C3!50}    SPIn-NeRF~\cite{mirzaei2023spin} & CVPR'23 & 10 & 100   & Images &  \begin{tabular}[c]{@{}c@{}} Real-world forward-facing
scenes with human annotated object masks \end{tabular} & Perception & \textcolor{blue}{2} \\

\rowcolor{C3!50}    LERF~\cite{kerr2023lerf} & ICCV'23 & 13 & -   & Videos &  \begin{tabular}[c]{@{}c@{}} A mixture of in-the-wild and posed long-tail scenes\end{tabular}  & Perception & \textcolor{blue}{5} \\

\rowcolor{C3!50}    Replica~\cite{straub2019replica}  &arXiv'19  & 18 &  -   &  Videos & \begin{tabular}[c]{@{}c@{}}  Highly photo-realistic 3D indoor scene dataset at room and building scale\end{tabular} & Perception & \textcolor{blue}{14} \\

\rowcolor{C3!50}    KITTI~\cite{geiger2012we}  &CVPR'12  & 22 &  -   &  Videos & \begin{tabular}[c]{@{}c@{}}   A city-scale dataset created for autonomous driving research\end{tabular} & Perception & \textcolor{blue}{5} \\

\rowcolor{C2!50}    Objaverse 1.0~\cite{deitke2023objaverse} & CVPR'23 & 818k &   -   & 3D objects &  \begin{tabular}[c]{@{}c@{}} A large dataset of over 800K 3D models with descriptive captions, tags, and animations.\end{tabular} & Generation & \textcolor{blue}{2} \\

\rowcolor{C2!50}    OmniObject3D~\cite{wu2023omniobject3d} & CVPR'23 & 6k &   -   & 3D objects &  \begin{tabular}[c]{@{}c@{}} Real-scanned 3D object captured with both 2D and 3D sensors, providing textured meshes, \\point clouds, multi-view rendered images, and multiple real-captured videos.\end{tabular}  & \begin{tabular}[c]{@{}c@{}} Generation \&  Perception \\ \& Reconstruction \end{tabular}  & \textcolor{blue}{4} \\

\rowcolor{C1!50}     People-Snapshot~\cite{alldieck2018video} & CVPR'18 & 24 &    1  & Videos &  \begin{tabular}[c]{@{}c@{}} Containing subjects captured with varying sets of garments \\ and with three different background scenes \end{tabular} & Virtual Humans & \textcolor{blue}{7} \\

\rowcolor{C1!50}     DynaCap~\cite{habermann2021real} & ToG'21 & 5 &    50-101  & Videos &  \begin{tabular}[c]{@{}c@{}} Recording 5 subjects wearing different types of apparel \\ and performing a wide range of motions like "dancing"\end{tabular} & Virtual Humans & \textcolor{blue}{1} \\

\rowcolor{C1!50}     ZJU-Mocap~\cite{peng2021neural} & CVPR'21 & 9 &    21  & Videos &  9 dynamic
human videos with 60 to 300 frames & Virtual Humans  & \textcolor{blue}{9} \\

\rowcolor{C1!50}     THuman4~\cite{zheng2022structured} & CVPR'22 & 3 &    24  & Videos &  multi-view
human videos ranging from 2500 to 5000 frames & Virtual Humans & \textcolor{blue}{3} \\

\rowcolor{C1!50}     NeuMan~\cite{jiang2022neuman} & ECCV'22 & 6 &    1  & Videos &  \begin{tabular}[c]{@{}c@{}} Monocular videos featuring a single individual \\ captured using a mobile phone \end{tabular}  & Virtual Humans & \textcolor{blue}{1} \\

\rowcolor{C1!50}     ActorsHQ~\cite{icsik2023humanrf} & arXiv'23 & 16 &    160  & Videos &  \begin{tabular}[c]{@{}c@{}} Containing 8 actors with casual clothing such as skirts or shorts\end{tabular}  & Virtual Humans & \textcolor{blue}{2}
\\ \bottomrule[1.5pt]
\end{tabular}%
}\label{dataset}
\vspace{-0.5cm}
\end{table*}

==> Tables/datasetV1_response.tex <==
\begin{table*}[htbp]
\centering
\caption{List of commonly used datasets for 3D Gaussians.}
\resizebox{\textwidth}{!}
{%
\begin{tabular}{lccccccc}
\toprule[1.5pt]
\rowcolor{C7!50}Dataset        & Year & Samples        & Camera Views & Type              & Description   & Task    & \#Number                              \\ \midrule[1pt]
 
\rowcolor{C6!50}  Mip-NeRF 360~\cite{barron2022mip}  &CVPR'22  & 9 & 360 viewpoint     & Videos & \begin{tabular}[c]{@{}c@{}}Outdoor and indoor scene containing a complex \\central object or area with a detailed background  \end{tabular} & Representation \& Reconstruction  & 49 \\

\rowcolor{C6!50}  Tanks and Temples~\cite{knapitsch2017tanks} & ToG'17 & 14 &   263-1107   & Videos & \begin{tabular}[c]{@{}c@{}}Ground-truth captured by high quality \\industrial laser scanner\end{tabular} & Representation \& Reconstruction & 34 \\

\rowcolor{C6!50}  DeepBlending~\cite{hedman2018deep}  &TOG'18  & 19 &  12-418    & Images & \begin{tabular}[c]{@{}c@{}} Images with suicient variety of scene content \end{tabular} & Representation \& Reconstruction & 18 \\

\rowcolor{C6!50}  Plenoptic Video~\cite{li2022neural} & CVPR'22 & 6 &   21   & Videos & \begin{tabular}[c]{@{}c@{}} Captured daily events with challenging scene motions\end{tabular} & Representation \& Reconstruction & 3 \\

\rowcolor{C6!50}  D-Nerf~\cite{pumarola2021d}    & CVPR'21 & 8 & 360 viewpoint     &  Synthetic videos &   \begin{tabular}[c]{@{}c@{}} Animated objects with complex geometries \\  and non-Lambertian materials \end{tabular}  & Representation \& Manipulation  &  9 \\

\rowcolor{C6!50}    DyNeRF~\cite{li2022neural}  & CVPR'22  & 6  & 20   & Videos &  \begin{tabular}[c]{@{}c@{}} Time-synchronized and calibrated multi-view \\  videos that covers challenging 4D scenes \end{tabular}  & Representation & 3 \\

\rowcolor{C6!50}    NeRF-LLFF~\cite{mildenhall2019llff}  &  SIGGRAPH'19 & 8 & forward-facing views & images &  A subset of Real Iconic  & Representation & 11 \\

\rowcolor{C5!50}  RealEstate10k~\cite{zhou2018stereo}  &ToG'18 & about 80k &  -   & Videos & \begin{tabular}[c]{@{}c@{}}Video clips on YouTube shot from a moving camera\end{tabular} & Reconstruction  & 3 \\

\rowcolor{C5!50}  ACID~\cite{liu2021infinite}  &ICCV'21 & 765  &  -   & Videos & \begin{tabular}[c]{@{}c@{}} A dataset of aerial landscape videos\end{tabular} & Reconstruction  & 2 \\

\rowcolor{C5!50}  ShapeNet~\cite{chang2015shapenet}  &2015 & about 60k  &  50   & Synthetic images & \begin{tabular}[c]{@{}c@{}} A richly-annotated, large-scale dataset of 3D shapes\end{tabular} & Reconstruction & 1 \\

\rowcolor{C4!50}  Tensor4D~\cite{shao2023tensor4d}    & CVPR'23 & 4 & 1, 4, 12     & Videos &   \begin{tabular}[c]{@{}c@{}}Dynamic half-body human videos by four\\ sparsely positioned, fixed RGB cameras\end{tabular}   & Manipulation & 5 \\

\rowcolor{C4!50}  NeRF-DS~\cite{pumarola2021d}    & CVPR'23 & 7 & 2 forward-facing views  & Videos &   Dynamic specular dataset & Manipulation  & 2 \\

\rowcolor{C4!50}  CoNeRF~\cite{kania2022conerf}    & CVPR'22 & 7 &  -  & Videos &   Real face scenes   & Manipulation & 1 \\

\rowcolor{C4!50}  InterHand2.6M~\cite{moon2020interhand2}    & ECCV'20 & 36 &  80-140 & Videos &   \begin{tabular}[c]{@{}c@{}} 2.6M labeled single and \\ interacting hand frames \end{tabular}  & Manipulation  & 1 \\

\rowcolor{C3!50}   NVOS~\cite{ren2022neural} & ICCV'22 & 7 &   20-62   &  Images &  \begin{tabular}[c]{@{}c@{}}  Real-world front-facing scenes with annotated object masks based on LLFF\end{tabular}  & Perception  & 1 \\

\rowcolor{C3!50}    SPIn-NeRF~\cite{mirzaei2023spin} & CVPR'23 & 10 & 100   & Images &  \begin{tabular}[c]{@{}c@{}} Real-world forward-facing
scenes with human annotated object masks \end{tabular} & Perception & 2 \\

\rowcolor{C3!50}    LERF~\cite{kerr2023lerf} & ICCV'23 & 13 & -   & Videos &  \begin{tabular}[c]{@{}c@{}} A mixture of in-the-wild and posed long-tail scenes\end{tabular}  & Perception & 5 \\

\rowcolor{C3!50}    Replica~\cite{straub2019replica}  &arXiv'19  & 18 &  -   &  Videos & \begin{tabular}[c]{@{}c@{}}  Highly photo-realistic 3D indoor scene dataset at room and building scale\end{tabular} & Perception & 14 \\

\rowcolor{C3!50}    KITTI~\cite{geiger2012we}  &CVPR'12  & 22 &  -   &  Videos & \begin{tabular}[c]{@{}c@{}}   A city-scale dataset created for autonomous driving research\end{tabular} & Perception & 5 \\

\rowcolor{C2!50}    Objaverse 1.0~\cite{deitke2023objaverse} & CVPR'23 & 818k &   -   & 3D objects &  \begin{tabular}[c]{@{}c@{}} A large dataset of over 800K 3D models with descriptive captions, tags, and animations.\end{tabular} & Generation & 2 \\

\rowcolor{C2!50}    OmniObject3D~\cite{wu2023omniobject3d} & CVPR'23 & 6k &   -   & 3D objects &  \begin{tabular}[c]{@{}c@{}} Real-scanned 3D object captured with both 2D and 3D sensors, providing textured meshes, \\point clouds, multi-view rendered images, and multiple real-captured videos.\end{tabular}  & \begin{tabular}[c]{@{}c@{}} Generation \&  Perception \\ \& Reconstruction \end{tabular}  & 4 \\

\rowcolor{C1!50}     People-Snapshot~\cite{alldieck2018video} & CVPR'18 & 24 &    1  & Videos &  \begin{tabular}[c]{@{}c@{}} Containing subjects captured with varying sets of garments \\ and with three different background scenes \end{tabular} & Virtual Humans & 7 \\

\rowcolor{C1!50}     DynaCap~\cite{habermann2021real} & ToG'21 & 5 &    50-101  & Videos &  \begin{tabular}[c]{@{}c@{}} Recording 5 subjects wearing different types of apparel \\ and performing a wide range of motions like "dancing"\end{tabular} & Virtual Humans & 1 \\

\rowcolor{C1!50}     ZJU-Mocap~\cite{peng2021neural} & CVPR'21 & 9 &    21  & Videos &  9 dynamic
human videos with 60 to 300 frames & Virtual Humans  & 9 \\

\rowcolor{C1!50}     THuman4~\cite{zheng2022structured} & CVPR'22 & 3 &    24  & Videos &  multi-view
human videos ranging from 2500 to 5000 frames & Virtual Humans & 3 \\

\rowcolor{C1!50}     NeuMan~\cite{jiang2022neuman} & ECCV'22 & 6 &    1  & Videos &  \begin{tabular}[c]{@{}c@{}} Monocular videos featuring a single individual \\ captured using a mobile phone \end{tabular}  & Virtual Humans & 1 \\

\rowcolor{C1!50}     ActorsHQ~\cite{icsik2023humanrf} & arXiv'23 & 16 &    160  & Videos &  \begin{tabular}[c]{@{}c@{}} Containing 8 actors with casual clothing such as skirts or shorts\end{tabular}  & Virtual Humans & 2
\\ \bottomrule[1.5pt]
\end{tabular}%
}\label{dataset}
\end{table*}
